Understanding and taming SSD read performance variability: HDFS case study

In this paper we analyze the influence that lower layers (file system, OS, SSD) have on HDFS' ability to extract maximum performance from SSDs on the read path. We uncover and analyze three surprising performance slowdowns induced by lower layers that result in HDFS read throughput loss. First, intrinsic slowdown affects reads from every new file system extent for a variable amount of time. Second, temporal slowdown appears temporarily and periodically and is workload-agnostic. Third, in permanent slowdown, some files can individually and permanently become slower after a period of time. We analyze the impact of these slowdowns on HDFS and show significant throughput loss. Individually, each of the slowdowns can cause a read throughput loss of 10-15%. However, their effect is cumulative. When all slowdowns happen concurrently, read throughput drops by as much as 30%. We further analyze mitigation techniques and show that two of the three slowdowns could be addressed via increased IO request parallelism in the lower layers. Unfortunately, HDFS cannot automatically adapt to use such additional parallelism. Our results point to a need for adaptability in storage stacks. The reason is that an access pattern that maximizes performance in the common case is not necessarily the same one that can mask performance fluctuations.

==> myintro2.tex <==
\section{Introduction}

Layering is a popular approach to build big data processing systems and it is
particularly central to the design of storage stacks for big data systems. Even
the simplest designs involve lots of layers: a data-processing system (Hadoop,
Spark) processes data stored in a distributed file system (HDFS, GFS), which in
turn relies on an OS running a local file system (ext4) which, finally, manages
data on disks. Oftentimes, additional layers are used such as big data stores
(BigTable, HBase) that are layered on top of the distributed file systems. Such
layered architectures are in part responsible for the massive success and
diversity of data processing systems today because they encourage rapid
development by reusing existing functionality.


Regardless of the specific layers in a storage stack the goal of fully
utilizing the capabilities of the underlying storage remains equally important.
Layering makes this goal more challenging to achieve because each layer can
introduce potential performance bottlenecks as well as sources of performance
variability. Performance bottlenecks in upper layers can completely mask
sub-optimal performance behavior in lower layers. Moreover, layering
significantly complicates root-cause analysis of performance problems and this
can lead to blame being assigned to the wrong layer due to lack of information.


In this paper we perform a deep dive into the performance of a critical layer
in today's big data storage stacks, namely the Hadoop Distributed File System
(HDFS). We particularly focus on the influence that other layers have on HDFS'
ability to extract the maximum throughput that the underlying storage is
capable of providing.  We analyze and discover a number of software and
hardware bottlenecks, some surprising, that prevent HDFS from reaching maximum
performance. We focus on the read path of HDFS because it can easily become a
performance bottleneck for an application's input stage due to accessing
comparatively slower storage media. Subsequent stages of an application are
typically sped-up using in-memory storage techniques and are oftentimes
fast because they process less data than the input stage. 


Central to our exploration is the storage access pattern of a single HDFS read
request: single threaded, sequential access to large files (hundreds of
megabytes) using buffered IO. This access pattern is simple but tried and
tested and has remained unchanged since the beginnings of HDFS. It is
increasingly important to understand whether even a single HDFS read request
using this access pattern can extract by itself the maximum throughput that the
underlying storage can provide. As many big data processing systems are heavily
IO provisioned and the ratio of cores to disks reaches 1, relying on task-level
parallelism to generate enough parallel requests to saturate storage is no
longer sufficient. Moreover, relying on such parallelism is detrimental to
application performance since each of the concurrent read requests is served
slower than it would be in isolation. 


We start our analysis by identifying and removing software bottlenecks present
in other layers and that limit HDFS. These are compute bottlenecks introduced
by the processing frameworks, network bottlenecks introduced by the OS
configuration as well as performance interference caused by the local file
system. We show that with simple changes HDFS reads can fully utilize the
underlying storage. 


Having decoupled HDFS performance from software bottlenecks we are now able to
clearly identify and analyze several surprising hardware performance
bottlenecks and performance variability sources induced by device internals. We
focus on SSDs in this work. First, we find that the read throughput obtained
from reading the same file over time can significantly and irreversibly
decrease due to an increase in the per-request latency inside some SSDs. 
Importantly this occurs on a file-level and not for an entire device.
We call this permanent slowdown. Second, we find temporary and periodic read
throughput slowdown.  While this temporary slowdown bears the hallmarks of SSD
garbage collection we find, surprisingly, that it can occur even in the
complete absence of writes.  This temporary slowdown is also caused by an
increase in the per-request latency inside the drive. Third, we find that file
fragmentation at the file system level (ext4) introduces performance
variability and slowdown during reading from every different file system
extent. 


All of the above findings show that the HDFS read access pattern, while
generally sufficient to maximize SSD performance, can fail to do so in certain
cases. Normally, HDFS maximizes SSD performance during reads because its access
pattern provides enough opportunity to leverage the internal SSD parallelism.
When, as discussed above, latencies inside the drive increase, the same HDFS
read access pattern does not adapt by increasing the IO request-level
parallelism and this results in a throughput loss. With the help of the FIO
synthetic benchmark we further analyze several OS-based approach to compensate
for the throughput loss.

With experiments on 3 SSD based systems, we show that each of the slowdown we
identified can individually introduce at least 10\% read throughput
degradation. The effect is cumulative. In the worst case, all slowdowns can
overlap leading to a 30\% throughput loss.

The contributions of the paper are as follows:
\begin{itemize}

\item We decouple HDFS read performance from several compute and configuration
bottlenecks and show that it can maximize SSD read throughput. 

\item We identify and analyze the permanent slowdown affecting reads from the
same file over time.

\item We identify and analyze temporary slowdowns that affect reads even in the
absence of writes. 

\item We identify and analyze the fragmentation slowdown affecting reads
crossing to every new file system extent.  

\end{itemize}

 







==> setup.tex <==
\section{Experimental Setup and Workloads}

In this section, we describe the hardware and software set- tings, tools, 
baselines and workloads used for our analysis.

%Check if HW should be described on a table
\textbf{Hardware.} We evaluate our experiments on three types of machines. %Maybe a table will be better?
\textit{Machine A} has 2 Intel Xeon 2.4GHz E5-2630 processors, with 32 cores 
in total,  132GB of RAM, and a 450GB Intel SATA SSD (MLC).\todo{trex117}
\textit{Machine B} has 4 Intel Xeon 2.7GHz E5-4650 processors, with 32 cores 
in total, 1.5TB of RAM, and a 800GB HP \todo{(Double check with characteristics on email) fatnode}.
\textit{Machine C} has Intel Xeon 2.4GHz E5-2630 processors, with 32 cores 
in total,  132GB of RAM, and a 512GB Samsung SATA SSD (V-NAND).\todo{trex133}
%Machine A - Trex 117
%Machine B - Fatnode
%Machine C - New SSD in trex133

\textbf{Software.} We evaluate our expriments on the linux kernel version 4.4.0.
We evaluate our experiments on top of ext4, one of the mostly used linux 
file systems.
On the HDFS side we use version 2.7.1.

\textbf{Monitoring Tools.} To monitor IO at the storage device, we rely on
blktrace and blkparse. Blktrace collects IO information at the
block layer, while blkparse makes the traces human readable.
On the other hand, we use perf to monitor function calls.
We use strace to monitor system calls.

\textbf{Baselines.} %Might be better in methodology...
FIO - Sync, aio
sendFile toy program.
Not sure if this is a baseline, or if it should be 
part of the workload part .

\textbf{Workload.} We evaluate HDFS performance on a read workload. A WordRead 
workload, a WordCount without the Count. This way, we guarantee tha.
In order to separate computation for storage, that is count the words after 
everything has been read, we perform a bulk read of a large size (256MB), 
rather than having smaller word reads, and thus overlapping computation and 
reads. 
HDFS block size is 256MB, a size used by production installations of 
HDFS~\cite{misra2017Scaling,zhang2016history}.
8 blocks per file.

HDFS and Hadoop jars are kept in a different IO device. So that reads to them do
not affect our HDFS reads.
